Fault Localization from the Semantic Code Search Perspective

The software development process is characterized by an iterative cycle of continuous functionality implementation and debugging, essential for the enhancement of software quality and adaptability to changing requirements. This process incorporates two isolatedly studied tasks: Code Search (CS), which retrieves reference code from a code corpus to aid in code implementation, and Fault Localization (FL), which identifies code entities responsible for bugs within the software project to boost software debugging. These two tasks exhibit similarities since they both address search problems. Notably, CS techniques have demonstrated greater effectiveness than FL ones, possibly because of the precise semantic details of the required code offered by natural language queries, which are not readily accessible to FL methods. Drawing inspiration from this, we hypothesize that a fault localizer could achieve greater proficiency if semantic information about the buggy methods were made available. Based on this idea, we propose CosFL, an FL approach that decomposes the FL task into two steps: query generation, which describes the functionality of the problematic code in natural language, and fault retrieval, which uses CS to find program elements semantically related to the query. Specifically, to depict the buggy functionalities and generate high-quality queries, CosFL extensively harnesses the code analysis, semantic comprehension, and decision-making capabilities of LLMs. Moreover, to enhance the accuracy of CS, CosFL captures varying levels of context information and employs a multi-granularity code search strategy, which facilitates a more precise identification of buggy methods from a holistic view. The evaluation on 835 real bugs from 23 Java projects shows that CosFL successfully localizes 324 bugs within Top-1, which significantly outperforms the state-of-the-art approaches by 26.6%-57.3%.

==> algorithm/algorithm1.tex <==
\begin{center}
\begin{algorithm}[!t]
\caption{Eliminate undersized modules.} % algorithm name
\footnotesize
\SetCommentSty{emph}
\LinesNumbered %show line number
\label{algorithm1}
\KwIn{$N$: the minimal module size. $C$: All modules.} % args
\KwOut{$C$: The changed modules.} % output
$C'$ = getUndersizedModules($C$, $N$) \tcc*{Get modules in $C$ that smaller than $N$}
\For{$c'_i$ in $C'$}{
    $V$ = getNodes($C'$) \tcc*{All method nodes in $c'_i$}
    $c_{t}$ = None \tcc*{The target appropriate-size module for $c'_i$}
    $\epsilon = 0$ \tcc*{A variable to record the weight between the undersized and target module}
    \For{$c_i$ in $C - C'$}{
        $\epsilon' = 0$ \tcc*{Record the weight between two modules}
        \For{$v_i$ in $V$}{
            $C^*$ = getNeighbors($v_i$) \tcc*{Get all modules that have calling relationships with method $v_i$}
            \For{$C^*_i$ in $C^*$}{
                \If{$C^{*}_{i} == c_{i}$}{
                    $w$ = getWeight($v_i$,$C^*_i$) \tcc*{$w$ is the sum of edge weights between node $v_i$ and module $C^*_i$}
                    $\epsilon' += w$
                }
            }
        }
        \If{$\epsilon' > \epsilon$}{
            $\epsilon = \epsilon'$\;
            $c_{t} = c_i$
        }
    }
    \For{$v_i$ in $V$}{
        $c_{t}$.addNode($v_i$)\;
        $c'_i$.removeNode($v_i$)\;
    }
}
Return $C$
\end{algorithm}
\end{center}

==> prompts/prompt4.tex <==

\prompt{Prompt 4: Localization Result Refinement}{4}{
A bug in the codebase has caused one or more test cases to fail. Your task is to analyze a potentially suspicious method and determine its likelihood of being the source of the bug.\\

\vspace{-0.1cm}
\textbf{\# Given information}

Faulty Location Hypothesis: <The Result of Fault Analysis Phase>

One of the retrieved suspicious methods: <The Source Code and Comment of the Method>\\

\vspace{-0.1cm}
\textbf{\# Instructions}

1. Carefully examine the Faulty Location Hypothesis and the source code of the suspicious method.

2. Consider the following factors in your analysis:

\hspace{10pt}- How closely does the method's functionality align with the Faulty Location Hypothesis?
   
\hspace{10pt}- Are there any obvious issues or potential bugs in the method's implementation?

\hspace{10pt}- Does the method interact with components or data that could be related to the test failures?

\hspace{10pt}- Are there any error-prone patterns or anti-practices present in the code?

3. Evaluate the likelihood that this method is responsible for the test failure.

4. Provide a concise but thorough explanation for your assessment.

5. Assign a suspiciousness score to the method on a scale of 0.0 to 10.0, where:

\hspace{10pt}- 0.0 means the method is very unlikely to be the cause of the bug
   
\hspace{10pt}- 10.0 means the method is very likely to be the cause of the bug \\

\vspace{-0.1cm}
\textbf{\# Response Format}

The output should include the following sections:

\hspace{10pt}- REASON: A clear, concise explanation of your assessment.

\hspace{10pt}- SCORE: A suspiciousness score between 0.0 and 10.0, based on your evaluation.

}
